Deep RL Dual Sourcing Inventory Management with Supply and Capacity Risk Awareness

In this work, we study how to efficiently apply reinforcement learning (RL) for solving large-scale stochastic optimization problems by leveraging intervention models. The key of the proposed methodology is to better explore the solution space by simulating and composing the stochastic processes using pre-trained deep learning (DL) models. We demonstrate our approach on a challenging real-world application, the multi-sourcing multi-period inventory management problem in supply chain optimization. In particular, we employ deep RL models for learning and forecasting the stochastic supply chain processes under a range of assumptions. Moreover, we also introduce a constraint coordination mechanism, designed to forecast dual costs given the cross-products constraints in the inventory network. We highlight that instead of directly modeling the complex physical constraints into the RL optimization problem and solving the stochastic problem as a whole, our approach breaks down those supply chain processes into scalable and composable DL modules, leading to improved performance on large real-world datasets. We also outline open problems for future research to further investigate the efficacy of such models.

==> preamble.tex <==
% % Required packages
% \usepackage{amsmath,amsthm,amssymb,amsfonts,cancel}
% % \usepackage{amsmath,amsfonts}
% \usepackage{thmtools,enumitem,subfigure,xspace}

% \usepackage{tikz}
% \usetikzlibrary{bayesnet}
% \usetikzlibrary{arrows}

% % PAPER SPECIFIC MACROS
% \makeatletter
% \def\blfootnote{\xdef\@thefnmark{}\@footnotet   ext}
% \makeatother

% % \usepackage{tabulararray}

% \usepackage{makecell}

\usepackage{mathtools}
% \usepackage{dsfont}
% \usepackage{tcolorbox}
% %\usepackage{bbm}
% \usepackage{todonotes}
% \usepackage{tensor}
% \usepackage{caption}
% % \usepackage{subcaption}
% \usepackage{bm}
% \ifdefined\arxiv
% \usepackage[colorlinks=true,breaklinks=true,bookmarks=true,urlcolor=magenta,citecolor=magenta,linkcolor=magenta,bookmarksopen=false,draft=false]{hyperref}
% \else
% \usepackage{hyperref}
% \fi
% \usepackage{placeins}
% \usepackage[capitalize,noabbrev]{cleveref}


% \newenvironment{rproofof}[1]{ \ifdefined\informs \begin{proof}{\it Proof of #1.}
% \else \begin{proof} \fi }{ \ifdefined\informs 
% \Halmos \end{proof} \else \end{proof} \fi  }

% \newenvironment{rproof}{ \ifdefined\informs \proof{\it Proof.}
% \else \begin{proof} \fi }{ \ifdefined\informs 
% \Halmos \endproof \else \end{proof} \fi  }



\newcommand{\epi}{\mathrm{epi}}
\newcommand{\Rea}{{\Bbb R}}
\newcommand{\Int}{{\Bbb Z}}
\newcommand{\Rat}{{\Bbb Q}}
\newcommand{\Cmp}{{\Bbb C}}
\newcommand{\Nat}{{\Bbb N}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RR}{\mathbb{R}}
%\renewcommand{\S}{\mathcal{S}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\inv}{\texttt{Inv}\xspace}

% % PAPER SPECIFIC MACROS
% \makeatletter
% \def\blfootnote{\xdef\@thefnmark{}\@footnotet   ext}
% \makeatother

% \crefformat{section}{\S#2#1#3} % see manual of cleveref, section 8.2.1
% \crefformat{subsection}{\S#2#1#3}
% \crefformat{subsubsection}{\S#2#1#3}

\newcommand{\GuidedMAC}{\textsc{Hindsight MAC}\xspace}
\newcommand{\GuidedRL}{Hindsight Learning~}
\newcommand{\GuidedQD}{\textsc{Hindsight Q-Distillation}\xspace}
\newcommand{\DeltaIPGap}{\Delta^{\texttt{\dag}}}
\newcommand{\Qip}{Q^{\texttt{\dag}}}
\newcommand{\Vip}{V^{\texttt{\dag}}}

\newcommand{\MARO}{\texttt{MARO}\xspace}
\newcommand{\ORGym}{\texttt{OR-Gym}\xspace}
\newcommand{\pip}{\pi^{\texttt{\dag}}}
\newcommand{\perm}{\overline{\pi}^\star}
\newcommand{\ORSuite}{\texttt{ORSuite}\xspace}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\pstar}{\pi^\star}
\newcommand{\Exp}[1]{\mathbb E \left[ #1 \right]} % Variance
\newcommand{\BarExp}[1]{\overline{\mathbb E} \left[ #1 \right]}
\newcommand{\bfxi}{\boldsymbol \xi}
\newcommand{\PXi}{\mathcal{P}_{\Xi}}
\newcommand{\plan}{\textsc{Hindsight}}
\newcommand{\Regret}{\textsc{Regret}}

\mathchardef\mhyphen="2D % Define a "math hyphen"

\ifdefined \argmin
\else \DeclareMathOperator*{\argmin}{arg\,min}
\fi
\ifdefined \argmax
\else \DeclareMathOperator*{\argmax}{arg\,max}
\fi

% \DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
% \DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
% \DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\newcommand{\E}{\mathbb{E}}

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

\DeclareMathOperator*{\tsum}{\textstyle\sum}
\newcommand{\Ind}[1]{\mathds{1}_{\left[ #1 \right]}}

% \setlist[itemize]{leftmargin=*}

% %\usepackage{titlesec} % or RequirePackage[loadonly]{titlesec} in a cls file
% %\titleformat{\subsubsection}[runin]{\normalfont\bfseries}{\thesubsubsection.}{3pt}{}


% % \theoremstyle{plain}
% \newtheorem{assumption}{Assumption}
% \newtheorem{definition}{Definition}
% \newtheorem{theorem}{Theorem}%[section]
% \newtheorem{corollary}{Corollary}[theorem]
% \newtheorem{lemma}[theorem]{Lemma}


% % Add your name/color. Use \<name>edit{} for edits and \<name>comment{} for comments

% \usepackage[suppress]{color-edits}
% %\usepackage{color-edits}
% \addauthor{sb}{violet}
% \addauthor{srstodo}{blue}
% \addauthor{srs}{orange}
% \addauthor{ca}{purple}
% \addauthor{as}{violet}


